Urban Scene Diffusion through Semantic Occupancy Map

Generating unbounded 3D scenes is crucial for large-scale scene understanding and simulation. Urban scenes, unlike natural landscapes, consist of various complex man-made objects and structures such as roads, traffic signs, vehicles, and buildings. To create a realistic and detailed urban scene, it is crucial to accurately represent the geometry and semantics of the underlying objects, going beyond their visual appearance. In this work, we propose UrbanDiffusion, a 3D diffusion model that is conditioned on a Bird's-Eye View (BEV) map and generates an urban scene with geometry and semantics in the form of semantic occupancy map. Our model introduces a novel paradigm that learns the data distribution of scene-level structures within a latent space and further enables the expansion of the synthesized scene into an arbitrary scale. After training on real-world driving datasets, our model can generate a wide range of diverse urban scenes given the BEV maps from the held-out set and also generalize to the synthesized maps from a driving simulator. We further demonstrate its application to scene image synthesis with a pretrained image generator as a prior.

==> fig_tex/completion.tex <==
\begin{figure}[ht!]
\centering
\includegraphics[width = 1\linewidth]{fig/null.jpeg}
\label{fig:completion}
\end{figure}
    


==> fig_tex/diff_process.tex <==
\begin{figure}[ht!]


\includegraphics[width=1\linewidth,clip, trim = 50 50 400 170]{fig/diff_denoise_vis.pdf}

\caption{Diffusion process and denoising process on semantic occupancy map. The up row shows the diffusion process of input occupancy map data and the bottom row shows denoising process during generating samples. 

}
\label{fig:diff_proc}
\vspace{-3mm}
\end{figure}
    


==> fig_tex/diverse.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{fig/diverse_fig.pdf}
\caption{Diverse scenes generation. One BEV map could generate different scenes.}
    \label{fig:diverse}
\end{figure}


==> fig_tex/inpainting.tex <==
\begin{figure}[ht!]
\centering
\begin{subfigure}[b]{0.33\linewidth}
\includegraphics[width=1\linewidth]{fig/null.jpeg}
\caption{naive inpainting}
\end{subfigure}%
\begin{subfigure}[b]{0.33\linewidth}
\centering
\includegraphics[width=1\linewidth]{fig/null.jpeg}
\caption{Ours}
\label{subfig:ours}
\end{subfigure}%
\begin{subfigure}[b]{0.33\linewidth}
\centering
\includegraphics[width=1\linewidth]{fig/null.jpeg}
\caption{Reference}
\end{subfigure}%
\caption{inpainting compare}
\label{fig:inpainting}
\end{figure}
    


==> fig_tex/method_compare.tex <==
\begin{figure*}[ht!]
\centering
\begin{subfigure}[b]{0.19\linewidth}
\includegraphics[width=1\linewidth]{fig/null.jpeg}
\caption{condition~\cite{}}
\end{subfigure}%
\centering
\begin{subfigure}[b]{0.19\linewidth}
\includegraphics[width=1\linewidth]{fig/null.jpeg}
\caption{method1~\cite{}}
\end{subfigure}%
\begin{subfigure}[b]{0.19\linewidth}
\includegraphics[width=1\linewidth]{fig/null.jpeg}
\caption{method2~\cite{}}
\end{subfigure}%
\begin{subfigure}[b]{0.19\linewidth}
\centering
\includegraphics[width=1\linewidth]{fig/null.jpeg}
\caption{Ours}
\label{subfig:ours}
\end{subfigure}%
\begin{subfigure}[b]{0.19\linewidth}
\centering
\includegraphics[width=1\linewidth]{fig/null.jpeg}
\caption{Reference}
\end{subfigure}%
\caption{different methods compare}
\label{fig:method compare}
\end{figure*}
    


==> fig_tex/pair_data.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{fig/pair_data.png}
    \caption{Visualization of the paired data from nuScenes dataset~\cite{nuscenes}. The second row and third row are 2D semantic map and depth map separately, which are projected from 3D semantic occupancy maps. The final row shows the combination of semantic map and rgb images.}
    \label{fig:pair_data}
\end{figure}

==> fig_tex/supp_fig.tex <==
\begin{figure*}[ht!]
\centering

\includegraphics[width=1\linewidth]{fig/supp_fig_waymo_nuplan.pdf}


\vspace{-3mm}
\caption{Scenes generated from the BEV maps sampled from (a) the Waymo Motion Dataset\cite{waymo}  and (b) nuPlan Dataset~\cite{nuplan}. Even though our method do not utilize the data from waymo motion dataset and nuplan for training, we could also get reasonable scenes from these BEV maps.}
\label{fig:supp_fig}
\end{figure*}
    


==> fig_tex/supp_fig_synthesis.tex <==
\begin{figure*}[ht!]
\centering

\includegraphics[width=1\linewidth]{fig/img_fig.pdf}

\vspace{5mm}
\caption{Scenes synthesis on different generated samples. Our method ensures temporal consistency in the scene, thanks to the use of solid 3D representations. }
\label{fig:supp_fig_synthesis}
\end{figure*}
    


==> fig_tex/teaser.tex <==
\begin{figure*}[ht!]
\centering

\includegraphics[width=1\linewidth,clip, trim=0 0 0 0]{fig/teaser.pdf}
\caption{Diverse single-frame scenes and large-scale scenes generated by \NAME. The generated scene is represented by the semantic occupancy map, where the color labels indicate different semantic categories. The input BEV layout is also attached as a reference.} 
\label{fig:teaser}
\end{figure*}
    


==> files/tables/ablation_ae.tex <==
\setlength{\tabcolsep}{2.5pt}
\renewcommand\arraystretch{1.2}
\begin{table}[h] 
% \setlength{\abovecaptionskip}{-4pt}
% \setlength{\belowcaptionskip}{-4pt}
\vspace{-5mm}
\centering
\footnotesize

\begin{tabular}{lcc}
\toprule
Methods & IoU (\textuparrow)  & mIoU (\textuparrow)  \\ 
\toprule
VAE, KL & 0.982 & 0.682 \\
VQVAE, embed 512 &  0.987 & 0.764 \\ 
% VQVAE, embed 1024 (without ema + weighted loss)& 0.986 & 0.784 \\ 
VQVAE, embed 1024 with 1/4 resolution & \textbf{0.988} & 0.798 \\ 
VQVAE, embed 2048 with 1/8 resolution &  0.973 &  0.513 \\
VQVAE, embed 2048 with 1/4 resolution & \textbf{0.988} & \textbf{0.800} \\ 
\bottomrule
\end{tabular}
\caption{\textbf{Comparisons with different autoencoders.}  \bz{This table alone occupies too much space, maybe you can put it together with Tab~\ref{tab:ablation_cond} to make them more compact and save some space.}}

% \vspace{0.5mm}

\label{tab:ablation_ae}
 \vspace{-3mm}
\end{table}



==> files/tables/ablation_cfg_ddim.tex <==
\begin{table}[ht!]
\centering
\setlength{\tabcolsep}{12pt}
\vspace{-3mm}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|ccc|ccc}
\toprule
& \multicolumn{3}{c|}{Guidance scale} & \multicolumn{3}{c}{Inference steps} \\
& 2.5 & 5 & 10 & 50 & 100 & 150\\
\midrule
V-FID ($\downarrow$) & 275.2 & 291.4 & 302.1&295.6 & 291.4 & 290.2\\
MMD ($\downarrow$) &0.095 & 0.106 & 0.120& 0.110 & 0.106 & 0.103\\
\bottomrule
\end{tabular}
}
\caption{\textbf{Ablation for guidance scale and ddim steps.}}
\label{tab:ablation}
\vspace{-5mm}
\end{table}

==> files/tables/ablation_cond.tex <==
% \setlength{\tabcolsep}{2.5pt}
% \renewcommand\arraystretch{1.2}
\begin{table}[h] 
% \setlength{\abovecaptionskip}{-4pt}
% \setlength{\belowcaptionskip}{-4pt}
% \vspace{-5mm}
\centering

\setlength{\tabcolsep}{15pt}


\begin{tabular}{lcc}
\toprule
Methods & V-FID (\textdownarrow) & CC (\textuparrow) \\ 
\toprule
Crossattn & 311.3 &  0.252\\
Modulation &317.4 &  0.674\\
Concat &  \textbf{291.4 } & \textbf{0.789}\\ 
\bottomrule
\end{tabular}
\caption{\textbf{Comparisons with different condition options.} V-FID and CC (condition consistency) are reported as evaluation metrics.} 
\vspace{-10mm}
\label{tab:ablation_cond}
\end{table}



==> files/tables/ablation_diff.tex <==
\setlength{\tabcolsep}{2.5pt}
\renewcommand\arraystretch{1.2}
\begin{table}[ht!] 
% \setlength{\abovecaptionskip}{-4pt}
% \setlength{\belowcaptionskip}{-4pt}
%\vspace{-2mm}
\centering

\setlength{\tabcolsep}{15pt}
\caption{\textbf{Evaluation an comparisons with different autoencoder.} V-FID and CC (condition consistency) are reported as evaluation metrics.} 

\begin{tabular}{l|cc}
\toprule
Methods & V-FID & CC \\ 
\toprule
vq-reg & & \\
vq-kl &\checkmark &   \\ 
vq-quantized  & &   \\ 
\bottomrule
\end{tabular}

% \vspace{0.5mm}

\label{tab:baseline}
 \vspace{-3mm}
\end{table}



==> files/tables/baseline.tex <==
% \setlength{\tabcolsep}{2.5pt}
% \renewcommand\arraystretch{1.2}
\begin{table}[h] 
\centering
\setlength{\tabcolsep}{12pt}
\caption{\textbf{Quantitative comparisons with different baselines.} V-FID and MMD are reported as evaluation metrics.  }

\begin{tabular}{@{}lcc@{}}
\toprule
Methods &   V-FID (\textdownarrow)  & MMD (\textdownarrow)    \\ 
\toprule
2D-3D lifting &567.0 &  1.292 \\
% VQGAN ~\cite{taming} &   &&  \\ 
Diff w. 3D U-Net ~\cite{stablediff} & 445.6  &  0.273 \\ 
Ours & \textbf{291.4} & \textbf{0.106} \\
\bottomrule
\end{tabular}

% \vspace{0.5mm}

\label{tab:baseline}
 \vspace{-3mm}
\end{table}



==> files/tables/generate_urban_scene.tex <==
\begin{table}[ht]
    \centering
    \resizebox{1\linewidth}{!}{%
    \begin{tabular}{l|cccc}
    Urbanscenegeneration  & geometry & semantic  & large scale & appearance   \\
         &  & & & & 
    \end{tabular}
    }
    \caption{Comparison with other methods}
    \label{tab:method_comp}
\end{table}

==> files/tables/preference.tex <==


\begin{table}[ht!]
\centering
\setlength{\tabcolsep}{12pt}
\resizebox{1\linewidth}{!}{
\begin{tabular}{lc}
\toprule
Comparison & Preference \\
\midrule
Ours vs 2D-3D lifting & 100\% \\ 
Ours vs Diff w. 3D U-Net & 96.9\% \\
\bottomrule
\end{tabular}
}

\caption{\textbf{Human evaluation}}
\label{tab:human_eval}
\vspace{-7mm}
\end{table}
